SD-CPS: Taming the Challenges of Cyber-Physical Systems with a Software-Defined Approach

Cyber-Physical Systems (CPS) revolutionize various application domains with integration and interoperability of networking, computing systems, and mechanical devices. Due to its scale and variety, CPS faces a number of challenges and opens up a few research questions in terms of management, fault-tolerance, and scalability. We propose a software-defined approach inspired by Software-Defined Networking (SDN), to address the challenges for a wider CPS adoption. We thus design a middleware architecture for the correct and resilient operation of CPS, to manage and coordinate the interacting devices centrally in the cyberspace whilst not sacrificing the functionality and performance benefits inherent to a distributed execution.

==> background.tex <==
\section{Background}
\label{sec:background}





